Photometric Calibration of the First 1.5 Years of the Pan-STARRS1 Survey

We present a precise photometric calibration of the first 1.5 years of science imaging from the Pan-STARRS1 survey (PS1), an ongoing optical survey of the entire sky north of declination -30 degrees in five bands. Building on the techniques employed by Padmanabhan et al. (2008) in the Sloan Digital Sky Survey (SDSS), we use repeat PS1 observations of stars to perform the relative calibration of PS1 in each of its five bands, solving simultaneously for the system throughput, the atmospheric transparency, and the large-scale detector flat field. Both internal consistency tests and comparison against the SDSS indicate that we achieve relative precision of <10 mmag in g, r, and i_P1, and ~10 mmag in z and y_P1. The spatial structure of the differences with the SDSS indicates that errors in both the PS1 and SDSS photometric calibration contribute similarly to the differences. The analysis suggests that both the PS1 system and the Haleakala site will enable <1% photometry over much of the sky.

==> referee <==
> The paper evaluates the relative photometric calibration of the first 1.5 
> years of the Pan-Starrs1 (PS1) survey.
> The authors show that they achieve relative precision of about 1% in the 
> photometry.
> This is a thorough paper on a technical but important aspect of PS1, one of 
> the most ambitious current projects.
> The methodology is based on a previous calibration analysis
> of SDSS. The techniques would also be useful for other ongoing and future 
> large surveys.

> The paper should certainly be published in ApJ.
> I have however some comments. and I'd like therefore to ask the authors
> for minor modifications of their paper accordingly:

Thank you very much for the useful comments and encouragement!

Please find detailed responses to each of your comments below.

--
> 1) There is very little discussion (just a paragraph at the end of the paper)
> about the PS1 science.
> It would make sense to explain already in the introduction what are the 
> science requirements that lead to the demanding 1% accuracy in relative 
> photometry.
> Usually  modern surveys take a "designer's approach",
> defining the quality of photometry needed for particular science, so it is 
> surprising that there is so little discussion about this.
> For example, one would expect a different photometry requirement for time 
> variability of objects
> compared e.g. with a photometry over wide angular scales needed for large 
> scale structure studies.

We have added a paragraph to the introduction indicating some problems that require 1% photometric calibration.  As the referee points out, time-variability of objects is not really one of them; for these a local photometric calibration is probably a better choice.  For clustering studies over large angular scales, however, the photometric calibration can indeed be a dominant source of error (see Ross et al. 2012).

More generally, we find the fact that the stellar locus has ~10 mmag width (Ivezic et al. 2007) sufficient grounds for pursuing a calibration accurate to at least this level; otherwise photometric studies of stellar populations in the Galaxy must contend with large-spatial-scale errors if they wish to take full advantage of the narrowness of the stellar locus.  In my own work studying reddening at high Galactic latitudes, 10 mmag errors in the photometric calibration of the SDSS dominate the uncertainty in the reddening law.

New paragraph:
Current surveys require photometric calibration as accurate as possible, ideally to better than the percent level.  Typical photometric uncertainties from point-spread-function modeling reach the 1\% level, and absent an equally good photometric calibration, calibration errors will dominate this uncertainty.  Additionally, the width of the stellar locus is about 1\% in certain color combinations \citep{Ivezic:2007}, requiring an equally good calibration to allow stars to be photometrically identified most accurately.  Studies of the interstellar dust at high Galactic latitudes can be still more demanding; photometric calibration dominates the uncertainty in the analysis of \citet{Schlafly:2011}.  Uncertainty in the photometric calibration even at the 1\% level can contribute to significant variation in the number densities of galaxies used for clustering studies on large angular scales \citep{Ross:2012}.  In short, a number of current science projects are limited by photometric calibration accuracy.

> 2) The analysis is based on stars. Is there any problem of star-galaxy 
> separation? is there any problem of variability of some
> of the stars?

We have slightly modified the paragraph of section of 2.3 addressing star-galaxy separation.  Because we use only brightish objects and cut on aperture-psf magnitudes, the remaining galaxy contamination is very small and primarily contributes a small amount of noise to the fits.

> 3) It would be helpful to have the information on the PS1 filters (currently 
> in the text on page 2) placed in a Table.

We have added such a table.  We also changed the text slightly to agree with the table---the red cutoff of the y filter is rather broad, leading to some ambiguity as to its red cutoff.

> 4) Figures of sky projection: better to show in one of the standard equal 
> area projections.z

We have not done this.  For the purposes of this paper, adopting a rectangular projection in ra/dec is important, because the PS survey observes blocks of sky that are rectangular in ra/dec in chunks.  Accordingly, photometric calibration artifacts in PS data often have a telltale rectangular appearance in ra/dec, and adopting a Mollweide-like projection would act to conceal these artifacts.

We could of course adopt a rectangular equal-area projection, but these retain large angular distortions near the pole and make it harder to look up a part of the sky based on ra/dec.

As this is completely a matter of projection (internal to the analysis, we always pixelize in healpix), we have deemed it preferable to show maps that simplify looking up a particular ra/dec.

> 5) Could the calibration be improved if the data are divided into half-nights
> and third-nights
> (instead of nightly)?

Our adoption of nightly calibration parameters is largely driven by two things:
- inspection of calibration residuals on a per-night basis
- linking widely separated parts of the sky together

We have experimented with fitting a zero point per image rather than a zero point per night (i.e., ~few hundred parameters per night), and, when taken to that extreme, errors in the photometric calibration on large angular scales do become significant.  These can be in principle controlled with priors, but we haven't fully investigated this possibility.

Moreover, when we look at the photometric residuals on a per night basis (e.g., Figure 7), almost never do we see continuous trends over the course of the night.  Perhaps the only exception to this is a few nights in the y band, probably owing to changing humidity, which we have just thrown out.  Because the night is a natural time in the problem and because the system is stable on these time scales, we adopted this unit of time for the photometric calibration.

I have added a brief paragraph to section 2.3 explaining this.

New paragraph:
Other models for $Z$ could be adopted.  In principle we have enough information to fit a zero point for every \PS\ image independently, though this would greatly diminish the stability of the solution on large angular scales.  However, the \PS\ system has proven to be remarkably stable over the course of a night (\textsection \ref{subsec:nightlystability}), removing the need for a more finely grained calibration, and leading us to adopt a simple model fitting only two parameters per night.


